Exoplanet Occurrence Rate with Age for FGK Stars in Kepler

We measure exoplanet occurrence rate as a function of isochrone and gyrochronology ages using confirmed and candidate planets identified in Q1-17 DR25 Kepler data. We employ Kepler's pipeline detection efficiency to correct for the expected number of planets in each age bin. We examine the occurrence rates for planets with radii $0.2 \leq Rp \leq 20$ R$_\oplus$ and orbital periods $0.2 \leq P \leq 100$ days for FGK stars with ages between $1.5-8$ Gyr using the inverse detection efficiency method. We find no significant trend between occurrence rate and stellar ages; a slight, decreasing trend (within $1.5-2.5$ $\sigma$) only emerges for low-mass and metal-rich stars that dominate our sample. We isolate the effects of mass and metallicity on the occurrence rate trend with age, but find the results to be inconclusive due to weak trends and small sample size. Our results hint that the exoplanet occurrence rate may decrease over time due to dynamical instability from planet-planet scattering or planet ejection, but accurate ages and larger sample sizes are needed to resolve a clear relation between occurrence rate and age.

==> table_fit_params.tex <==
\begin{deluxetable}{c|c|c}
\tablecaption{The best fit parameters from this work and \cite{howard_2012} describing the trends in orbital period, planet radii and effective temperature.\label{tb:howard_results}}
\tablehead{\colhead{Parameter} & \colhead{This work} & \colhead{H12}} 
\startdata
$k_R$ & $89.40\pm30.26$ & $2.9^{+0.5}_{-0.4}$ \\
$\alpha$ & $-1.67\pm0.35$ & $-1.92\pm0.11$ \\
$k_P$ & $11.45\pm4.83$ & $0.035\pm0.023$\\
$\beta$ & $-0.06\pm0.13$ & $0.52\pm0.25$ \\
$P_0$ & $5.10\pm1.31$ & $4.8\pm1.6$\\
$\gamma$ & $1.85\pm0.47$ & $2.4\pm0.3$ \\
$f_0$ & $0.79\pm0.09$ & $0.165\pm0.011$\\
$k_T$ & $-0.38\pm0.17$ & $-0.081\pm0.011$ 
\enddata
\end{deluxetable}

==> table_slope_planet.tex <==
\begin{deluxetable*}{c|l|rccc}[t!]
\tablecaption{Slope and $p-$value for each distribution shown in Figure \ref{fig:planet_type} where the slope was calculated using Equation \ref{eq:lr}. Statistically significant results usually have a $p-$value below 0.05. \label{tb:slope_planet}}
\tablehead{Ages & Planet Type & Slope & $\sigma_\textrm{Slope}$ & $p-$value & Figure \\ 
& & Gyr$^{-1}$ & Gyr$^{-1}$ & & }
\startdata
Isochrone & Close & $-0.044$ & $0.002$ & $0.023$ & \ref{fig:planet_type}A \\
Isochrone & Far & $-0.013$ & $0.005$ & $0.242$ & \ref{fig:planet_type}A \\
Isochrone & Small & $-0.028$ & $0.021$ & $0.407$ & \ref{fig:planet_type}A \\
Isochrone & Big & $-0.012$ & $0.011$ & $0.475$ & \ref{fig:planet_type}A \\
Isochrone & Close--Small & $-0.037$ & $0.005$ & $0.079$ & \ref{fig:planet_type}C \\
Isochrone & Close--Big & $-0.003$ & $0.011$ & $0.854$ & \ref{fig:planet_type}C \\
Isochrone & Far--Small & $-0.002$ & $0.030$ & $0.948$ & \ref{fig:planet_type}C \\
Isochrone & Far--Big & $-0.004$ & $0.021$ & $0.889$ & \ref{fig:planet_type}C \\
Gyrochronology & Close & $0.009$ & $0.048$ & $0.879$ & \ref{fig:planet_type}B \\
Gyrochronology & Far & $-0.053$ & $0.032$ & $0.345$ & \ref{fig:planet_type}B \\
Gyrochronology & Small & $0.007$ & $0.030$ & $0.857$ & \ref{fig:planet_type}B \\
Gyrochronology & Big & $-0.058$ & $0.003$ & $0.031$ & \ref{fig:planet_type}B \\
Gyrochronology & Close--Small & $0.017$ & $0.043$ & $0.764$ & \ref{fig:planet_type}D \\
Gyrochronology & Close--Big & $-0.003$ & $0.014$ & $0.867$ & \ref{fig:planet_type}D \\
Gyrochronology & Far--Small & $0.017$ & $0.008$ & $0.278$ & \ref{fig:planet_type}D \\
Gyrochronology & Far--Big & $-0.083$ & $0.031$ & $0.230$ & \ref{fig:planet_type}D
\enddata
% \tablecomments{comments}
\end{deluxetable*}
\vspace*{-\baselineskip}
